Exploring Fine-tuning of the Next-to-Minimal Composite Higgs Model

We perform a detailed study of the fine-tuning of the two-site, 4D, Next-to-Minimal Composite Higgs Model (NMCHM), based on the global symmetry breaking pattern $SO(6)\rightarrow SO(5)$. Using our previously-defined fine-tuning measure that correctly combines the effect of multiple sources of fine-tuning, we quantify the fine-tuning that is expected to result from future collider measurements of the Standard Model-like Higgs branching ratios, in addition to null searches for the new resonances in the model. We also perform a detailed comparison with the Minimal Composite Higgs Model, finding that there is in general little difference between the fine-tuning expected in the two scenarios, even after measurements at a high-luminosity, 1 TeV linear collider. Finally, we briefly consider the relationship between fine-tuning and the ability of the extra scalar in the NMCHM model to act as a dark matter candidate, finding that the realisation of a $Z_2$ symmetry that stabilises the scalar is amongst the most natural regions in the parameter space, regardless of future collider measurements.

==> tex/Tuning.tex <==

\section{Fine-tuning in Many Observables}
\label{tuning}

Including a composite Higgs sector is a well-established method of raising the scale of natural new physics above $1$TeV. Partial compositeness of the heaviest flavour of quarks and leptons goes further to raise this scale without unsatisfying fine tuning. To consistently deal with fine-tuning comparisons between models, we would like to explore a measure that extends the usual concept of tuning to one that consistently considers every source of tuning $\Delta$. The amount of fine tuning in any particular parameter $x_i$ to produce the observable $\mathcal{O}$ has historically been that introduced by Barbieri and Giudice,
\begin{align}
\Delta_{BG,i}^\mathcal{O} = \Delta_{BG}^\mathcal{O}(x_i) = \abs*{\frac{x_i}{\mathcal{O}}\frac{\partial \mathcal{O}}{\partial x_i}}_{\mathcal{O}=\mathcal{O}_\textnormal{exp}}\label{BG}\, ,
\end{align}
%
where we use the definitions from the previous section. This gives a measure of fine tuning for each parameter. To find the total fine-tuning in $\mathcal{O}$, $\Delta^\mathcal{O}(\vec{x})$, one might simply take the maximum of all the $\Delta_{BG,i}$. Alternatively, one may define a vector of BG measures $\nabla^{\mathcal{O}_a}$ in the intuitive way, 
%
\begin{align}
\nabla^{\mathcal{O}_a} &= \left(\begin{matrix}
\Delta_{BG,1}\\
\Delta_{BG,2}\\
...\\
\Delta_{BG,n_p}
\end{matrix}\right)
\end{align}
%
and take the magnitude of this vector over $n_p$ parameters
\begin{align}
\Delta^\mathcal{O}(\vec{x}) = \sqrt{\sum\limits_i^{n_p} (\Delta_{BG,i})^2} = |\nabla^{\mathcal{O}_a}| \label{firstorder}\, .
\end{align}
%
%\marginpar{\footnotesize{n.b. Why magnitude for params, average for observables?}}
%
Similarly, to extend to $n_o$ observables, $\{\mathcal{O}_a\}$, we can average over each fine-tuning
\begin{align}
\Delta_1 = \frac{1}{n_o}\sum\limits_{a=1}^{n_o}\Delta^{\mathcal{O}_a}\, .
\end{align}
%
This has been the state-of-the art until recently. However, as pointed out by \cite{Barnard:2015ryq}, it is often the case that these fine-tuning vectors are not aligned. That is, the fine-tuning may come from more than one source and the fine-tuning measure should reflect this special double tuning - a higher order tuning. If they are completely orthogonal, then the higher order tuning should be simply the product of each single tuning. If they are completely parallel, the higher tuning should disappear. 

For any two particular tuning vectors $\{\nabla^{\mathcal{O}_a},\nabla^{\mathcal{O}_b}\}$, a quantity displaying these criteria is 
%
\begin{align}
\Delta_2^{ab} = \begin{vmatrix}
\nabla^{\mathcal{O}_a}\cdot\nabla^{\mathcal{O}_a} & \nabla^{\mathcal{O}_a}\cdot \nabla^{\mathcal{O}_b}\\
\nabla^{\mathcal{O}_a}\cdot\nabla^{\mathcal{O}_b} & \nabla^{\mathcal{O}_b}\cdot \nabla^{\mathcal{O}_b}
\end{vmatrix}^\frac{1}{2}_{\mathcal{O}=\mathcal{O}_\textnormal{exp}\, .}\label{double}
\end{align}
%
For orthogonal tunings, $\nabla^{\mathcal{O}_a}\cdot \nabla^{\mathcal{O}_b}\rightarrow 0$ and thus $\Delta_2^{ab} \rightarrow \nabla^{\mathcal{O}_a} \nabla^{\mathcal{O}_b}$. For aligned tunings $\nabla^{\mathcal{O}_a} = \lambda \nabla^{\mathcal{O}_b}$, then $\nabla^{\mathcal{O}_a}\cdot \nabla^{\mathcal{O}_b}\rightarrow \lambda \nabla^{\mathcal{O}_a} \nabla^{\mathcal{O}_a}$ and thus $\Delta_2^{ab} \rightarrow 0$. Noting that Equation~\ref{double} is the area spanned by any two tuning vectors, this behaviour should be intuitive. 

The total fine tuning $\Delta_2$ should then fulfil the criteria that (i) for all observables independent it be a maximum, (ii) for only one independent observable it vanish, and (iii) for the limiting case of two independent observables, it simply be the single double-tuning measure. For three observables, the measure satisfying these is 
\begin{align}
\Delta_2 = \frac{1}{2}(\Delta_2^{ab} +\Delta_2^{bc}+\Delta_2^{ca})\, .\label{totaldouble}
\end{align}
One can see that for observable $c$ proportional to $b$, $\mathcal{O}_c = \kappa \mathcal{O}_b$, then $\Delta_2^{bc}\rightarrow 0$ and $\Delta_2^{ac} \rightarrow \Delta_2^{ab}$. This comes from both Eq. (\ref{double}) disappearing for aligned tunings, and Eq. (\ref{BG}) being insensitive to a scaling $\kappa$.  Thus, $\Delta_2$ behaves as we would like. For more than three observables, the third criterion is not unique. In particular, for four and five observables, there are two configurations for, e.g. observables $a$ and $b$ to be independent. Configuration 1 has all dependency on one observable, configuration 2 has the dependency shared across variables, shown in figure \ref{configs}.

\begin{figure}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=0.4\linewidth]{configa}
\caption{We have one set of dependencies \\ $\mathcal{O}_a = \kappa_1\mathcal{O}_b = \kappa_2 \mathcal{O}_d$}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=0.4\linewidth]{configb}
\caption{We have two dependencies $\mathcal{O}_a = \kappa_1\mathcal{O}_b$ and $\mathcal{O}_c = \kappa_2 \mathcal{O}_d$}
\end{subfigure}
\caption{The configurations available for one source of double-tuning amongst four observables}
\label{configs}
\end{figure}
Configuration 1 algebraically satisfies criterion (iii) in a simple extension of Eq. (\ref{totaldouble}) to unordered pairs over $n_o$ observables
%
\begin{align}
\Delta_2 &= \frac{1}{n_o-1} \sum\limits_{\{\,a,b\,\} | b<a}^{\binom{n_o}{2}} \Delta_2^{ab}\label{gendoubletotal}\, .
\end{align}
%
However, calculating Eq. (\ref{gendoubletotal}) for configuration 2 gives more unordered pairs, and thus a factor of $4/3$ above configuration 1. This is the limit of inaccuracy in Equation~\ref{gendoubletotal}, but for randomly distributed observables the correction drops to $ <10 \% $ typically. For the purposes of fine-tuning being an order of magnitude calculation, we will accept this measure as a good approximation.

The generalisation of Equation~\ref{double} to three observables is also quite straightforward, where we take the volume spanned by three particular tuning vectors:
%
\begin{align}
\Delta_3^{abc} &= \begin{vmatrix}
\nabla^{\mathcal{O}_a}\cdot\nabla^{\mathcal{O}_a} & \nabla^{\mathcal{O}_a}\cdot \nabla^{\mathcal{O}_b} &\nabla^{\mathcal{O}_a}\cdot \nabla^{\mathcal{O}_c} \\\nabla^{\mathcal{O}_a}\cdot\nabla^{\mathcal{O}_b} & \nabla^{\mathcal{O}_b}\cdot \nabla^{\mathcal{O}_b} &\nabla^{\mathcal{O}_b}\cdot \nabla^{\mathcal{O}_c}\\\nabla^{\mathcal{O}_a}\cdot\nabla^{\mathcal{O}_c} & \nabla^{\mathcal{O}_b}\cdot \nabla^{\mathcal{O}_c} &\nabla^{\mathcal{O}_c}\cdot \nabla^{\mathcal{O}_c}
\end{vmatrix}^\frac{1}{2}_{\mathcal{O}=\mathcal{O}_\textnormal{exp}}\, . \label{triple}
\end{align}
%
Being a volume, this follows the same behaviour as the double tuning derived above. We sum various triple tunings with the extension
%
\begin{align}
\Delta_3 &= \frac{1}{n_o-2} \sum\limits_{\{\,a,b,c\,\} | c<b<a}^{\binom{n_o}{3}} \Delta_3^{abc}\, .
\end{align}
%
In general, the $N$-th order of tuning of a set of $N$ particular observables $\bm{\nabla}_N=(\nabla^{\mathcal{O}_a},\nabla^{\mathcal{O}_b},...)$ is given by 
%
\begin{align}
\Delta^{ab...}_N = |\bm{\nabla}_N^T \cdot\bm{\nabla}_N|^{\frac{1}{2}}
\end{align}
%
and the $N$-th higher order tuning over \textit{all} $n_o$ observables is 
%
\begin{align}
\Delta_N &= \frac{1}{n_o-(N-1)} \sum\limits_{\{\,a,b,...\,\} | ...<b<a}^{\binom{n_o}{N}} \Delta_N^{ab...}\, .
\end{align}
%
Finally, we simply sum each order of tuning for a measure of higher order tuning:
%
\begin{align}
\Delta = \sum_{i=1}^{n_o} \Delta_i\, .
\end{align}
%
This is the measure by which we evaluate the success of each leptonic embedding in improving the naturalness of the MCHM. Before stating and comparing our results with those of previous studies~\cite{carmona2015,Barnard:2015ryq}, it must be noted that our new measure will give larger absolute numbers for the fine tuning. To see why, consider three factors: arbitrary increase of parameters, arbitrary increase of observables, and genuinely more sensitive expressions (i.e. compare the general double tuning of Higgs mass/vev to the double tunings of the new observables). For random fine-tuning vectors, we would expect the following general dependencies. 

At order one of tuning, the number of observables $N$ will not affect the measure as they are averaged out. In terms of $n_p$ from equation \ref{firstorder}, $\Delta^\mathcal{O}$ goes as 
\begin{align}
\Delta^\mathcal{O} \sim \sqrt{n_p}\, .
\end{align}
%
At order two of higher order tuning - that is, double fine tuning - the measure goes as (Equations \ref{double} and \ref{totaldouble}):
\begin{align}
\Delta_2 &\propto \frac{1}{n_o -1}\left(\begin{matrix}
n_o\\
2
\end{matrix}\right) = \frac{n_o!}{(n_o - 1)2!(n_o-2)!}=\frac{n_o}{2}\sim n_o\, ,\\
\Delta_2 &\propto \begin{vmatrix}
\nabla_a \cdot \nabla_a & \nabla_a \cdot \nabla_b\\
\nabla_a \cdot \nabla_b & \nabla_b \cdot \nabla_b
\end{vmatrix}^{1/2} \sim \sqrt{\nabla_a^2 \nabla_b^2} \sim n_p\, .
\end{align}
%
assuming mostly orthogonal observables. That is, at second order, the measure scales linearly with number of both parameters and observables. At third order, the measure goes as 

\begin{align}
\label{tripletuning}
\Delta_3 &\propto \frac{1}{n_o -1}\left(\begin{matrix}
n_o\, ,\\
2
\end{matrix}\right) \sim n_o^2\\
\Delta_3 &\propto n_p^{3/2}\, .
\end{align}

Higher orders $\Delta_N$ follow this pattern of $\sim n_o^{N-1},n_p^{N/2}$. Of course there is a further scaling of the measure when considering higher numbers of observables. When going from three to four observables, not only do we increase the fine tuning out-of-hand by $(4/3)^2 \approx 1.8$, we also add in the possibility of order-four tuning, which is generically a factor of $\Delta_1$ greater than order-three. 

Considering all of these artefacts of the tuning measure, we arrive at a generic increase from \cite{Barnard:2015ryq} to this paper of\footnote{We remind the reader that Barnard, White have three observables and nine parameters}
\begin{align}
\textnormal{factor} &\approx	\left(\frac{5}{3}\right)^{(5-1)} \cdot \left(\frac{27}{9}\right)^{(5/2)} = 120\, .
\end{align}


